Reasoning about Weak Isolation Levels in Separation Logic

Consistency guarantees among concurrently executing transactions in local- and distributed systems, commonly referred to as isolation levels, have been formalized in a number of models. Thus far, no model can reason about executable implementations of databases or local transaction libraries providing weak isolation levels. Weak isolation levels are characterized by being highly concurrent and, unlike their stronger counterpart serializability, they are not equivalent to the consistency guarantees provided by a transaction library implemented using a global lock. Industrial-strength databases almost exclusively implement weak isolation levels as their default level. This calls for formalism as numerous bugs violating isolation have been detected in these databases. In this paper, we formalize three weak isolation levels in separation logic, namely read uncommitted, read committed, and snapshot isolation. We define modular separation logic specifications that are independent of the underlying transaction library implementation. Historically, isolation levels have been specified using examples of executions between concurrent transactions that are not allowed to occur, and we demonstrate that our specifications correctly prohibit such examples. To show that our specifications are realizable, we formally verify that an executable implementation of a key-value database running the multi-version concurrency control algorithm from the original snapshot isolation paper satisfies our specification of snapshot isolation. Moreover, we prove implications between the specifications -- snapshot isolation implies read committed and read committed implies read uncommitted -- and thus the verification effort of the database serves as proof that all of our specifications are realizable. All results are mechanized in the Rocq proof assistant on top of the Iris separation logic framework.

==> lstcoq.tex <==
%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{coq} {
% Comments may or not include Latex commands
texcl=false,

% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, From, Let, Ltac, Fixpoint, CoFixpoint, Add, Morphism, Relation,
Implicit, Arguments, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Context, Class, Global, Instance, Program, Infix,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Extern, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside, outside, Eval,
Check},

% Gallina
morekeywords=[2]{match, with, end, if, then, else, let, fst, snd, val, rec, Fork},
%morekeywords=[2]{forall, exists, exists2, fun, fix, cofix,
%      match, with, end, as, in, return, let, is, if, then, else,
%      for, of, nosimpl},

% Sorts
morekeywords=[3]{Set, Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
%morekeywords=[4]{
%         pose, set, move, case, elim, apply, clear,
%            hnf, intro, intros, generalize, rename, pattern, after,
%	    destruct, induction, using, refine, inversion, injection,
%         rewrite, congr, unlock, compute, field, fourier,
%            replace, fold, unfold, change, cutrewrite, simpl,
%         have, suff, wlog, suffices, without, loss, nat_norm,
%            assert, cut, trivial, revert, bool_congr, nat_congr,
%	 symmetry, transitivity, auto, split, left, right, autorewrite},        

% Terminators
%morekeywords=[5]{
%         by, done, exact, tauto, romega, omega,
%         assumption, solve, contradiction, discriminate},


% Control
%morekeywords=[6]{do, last, first, try, idtac, repeat},

morestring=[b]{"},

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% Size of tabulations
tabsize=3,							

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style for listings
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,							

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black!70!green!90}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{black!70!green!90}},
keywordstyle=[2]{\ttfamily\color{black!70!green!90}},
keywordstyle=[3]{\ttfamily\color{black!70!green!90}},

%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily\color{black!70!green!90},

% Style for comments
commentstyle={\itshape\color{gray}},

moredelim=[is][\color{black}]{@@}{@},
}

